Memtrade: A Disaggregated-Memory Marketplace for Public Clouds

We present Memtrade, the first memory disaggregation system for public clouds. Public clouds introduce a set of unique challenges for resource disaggregation across different tenants, including security, isolation and pricing. Memtrade allows producer virtual machines (VMs) to lease both their unallocated memory and allocated-but-idle application memory to remote consumer VMs for a limited period of time. Memtrade does not require any modifications to host-level system software or support from the cloud provider. It harvests producer memory using an application-aware control loop to form a distributed transient remote memory pool with minimal performance impact; it employs a broker to match producers with consumers while satisfying performance constraints; and it exposes the matched memory to consumers as a secure KV cache. Our evaluation using real-world cluster traces shows that Memtrade provides significant performance benefit for consumers (improving average read latency up to 2.8x) while preserving confidentiality and integrity, with little impact on producer applications (degrading performance by less than 2.1%).

==> discussion.tex <==
\section{Discussion}

\subsection{Network Stack}
As public cloud environments are typically virtualized, inter-VM
networking incurs additional latency due to traversing both kernel and
hypervisor networking stacks.  As shown in Figure~\ref{fig:latency},
kernel-bypass networking (\eg, DPDK, RDMA) offers lower latency in
virtualized environments; with RDMA and SR-IOV, the additional
overhead is minimal compared to bare-metal machines.  Unfortunately,
RDMA is not widely available in existing public clouds. While DPDK is
slower than RDMA, it still achieves single-digit $\mu s$ latencies for
small objects.  However, it consumes an excessive amount of CPU due to
polling (nearly 100\% of local CPU for larger objects), which
would require producers to have extremely idle CPU resources to be
practical.
% (97.51\% and 100\% of local CPU for 4~KB and 2~MB packets, respectively).
% In order to use DPDK, besides having sufficient memory
% to harvest, the producer needs sufficient idle CPU resources too.

Because of its universal availability, \spotframework currently uses
TCP networking, despite its relatively high overhead and other
limitations.  For deployments in private clouds, replacing TCP with
RDMA would improve performance significantly.

% Although TCP incurs a relatively larger overhead, in \spotframework,
% we consider it as the default underlying network stack, because of its
% wide availability.  Obviously, simply replacing TCP with RDMA (\eg, in
% a private cloud) can provide a significant performance boost for
% \spotframework.
%
% \mosharaf{TCP limits how small a value we can consider. Should we comment on that?}

\begin{figure}[!t]
  \centering
  \includegraphics[scale=0.6]{analysis/network-stack-latency.pdf}
  % \caption{Network latency for reading objects of different sizes, with kernel and hypervisor bypass.}
  \caption{Network latency using VMs vs. bare-metal hosts for various protocols and different object sizes.}
  \label{fig:latency}
\end{figure}

\subsection{Pricing Spot Memory}
\label{sec:price-model}

%Spot memory must be offered at a price that is attractive to both
%producers and consumers, providing incentives to participate in the
%spot-memory market.  A producer must weigh the cost of providing
%memory, including the risk of transient application performance
%degradation, against the monetary benefit of receiving income for
%otherwise-wasted resources, which can help defray the expense of
%running its own VM.  A consumer must weigh the monetary cost of
%leasing spot memory against the value of its expected performance
%benefit.
% from access to remote memory.

Numerous approaches inspired by microeconomics have been used to
determine prices for computational resources within individual
servers~\cite{ginseng1,ginseng2,currentcy}, distributed
systems~\cite{spawn,popcorn,g-commerce}, and the public
cloud~\cite{agmon2013deconstructing,raas,song2012optimal,zheng2015bid,xu2013dynamic,zhang2011dynamic}.
Typically, producers hold auctions designed to maximize profits, and
consumers employ bidding strategies to maximize utility.

\paragraph{Leveraging Spot-Instance Prices.}

In the public cloud, an alternative to spot memory is spinning up an
entire VM as a spot instance, and utilizing its memory
remotely~\cite{spot-cache}.  This provides a useful upper bound on the
reasonable price that can be charged for spot memory; higher prices
would present an arbitrage opportunity, making it profitable to rent
spot instances and resell their memory capacity as spot
memory.\footnote{This is analogous to breaking up a company when the
  sum of its parts is more valuable than the whole; instance CPU
  time could be resold as well.}

This observation suggests one simple method for setting a single
global price for spot memory dynamically -- without the complexity of
running separate auctions -- by leveraging price information in the
existing spot-instance market.  For example, the price for leasing $M$
MB of spot memory for $T$ minutes could be set to a fraction (such as
one-quarter) of the current cost of a spot instance for the same
duration, scaled by the ratio of $M$ to the instance's total memory
capacity.

\paragraph{Consumer Strategy.}

In general, it may be difficult for a consumer to estimate the
monetary value it should assign to additional memory.  However, when
its application is a cache, quantitative metrics can help guide this
estimate.  For example, lightweight sampling-based techniques~\cite{SHARDS,kinetic,cachesims} 
%such as
%SHARDS~\cite{SHARDS}, AET~\cite{kinetic}, or miniature
%simulation~\cite{cachesims} 
can estimate miss ratio curves (MRCs)
accurately, yielding the expected performance benefit from a larger
cache size.

The monetary value of additional cache space can be estimated by first
computing the current {\em price-per-hit} from the known cost to the
consumer of running its VM, and its observed hit rate.  The expected
increase in hits can be computed from an MRC, and valued based on the
per-hit price.  When spot memory is more valuable to the consumer than
its cost at the current market price, it should be leased, yielding an
economic consumer surplus.

The consumer must also consider the lower performance of a hit to
remote spot memory, relative to a local hit. For example, if this
increases the end-to-end latency observed by a client of the
cache significantly, the consumer may be willing to pay only a
fraction of its cost for a local hit.
% , depending on its actual QoS requirements.

%% XXX [carl] cut since too long and complex; simplified/shortened above
%%
%% Even without using MRCs, the cache can track the number of accesses to
%% a small sampled subset of its keys.  Whenever sampled entries are
%% evicted, their observed hit rates (access count divided by time
%% resident in the cache) can be smoothed to estimate the expected
%% marginal hit rate for an additional cache entry.  The monetary cost of
%% a marginal cache entry can be computed from the known price paid to
%% run the entire VM, scaled by the ratio of the size of a single entry
%% to the VM's total size.  Combining these values yields the marginal
%% {\em price-per-hit}, which can be used to decide if the current price
%% of spot-memory is attractive.\footnote{Since cache miss rates
%%   generally decrease monotonically with cache size, extrapolating from
%%   the per-entry value will overestimate the value of adding a large
%%   amount of cache space, which is better approximated using
%%   an MRC.  The {\em average} price-per-hit across the entire cache may
%%   also be useful.}  The residency time can also serve as an estimate
%% of the desired lease time to request for spot-memory allocations.

%% A similar calculation could be made to estimate the monetary cost
%% incurred for servicing a miss.

%% XXX [carl] some text about ghost buffers that might be useful
%%
%% Consider the case where the consumer is a key-value store that locally
%% stores ``proxy'' entries, as described in
%% Section~\ref{sec:security-design}.  Each proxy entry contains a key
%% and an associated value consisting of compact metadata that is used to
%% retrieve the larger actual value stored in remote spot memory.  These
%% proxy entries can also be viewed as {\em ghosts} -- small
%% metadata-only entries containing keys, but not actual values -- which
%% serve as placeholders to determine when an access would have been a
%% hit in a larger cache~\cite{tip-ghost}.

\paragraph{Early Reclamation.}

A consumer leases a fixed amount of spot memory from a producer for a
specified duration.  However, a producer may reclaim spot memory that
has been harvested from it at any time, in order to prevent
non-trivial performance degradation if its memory demand spikes.
While this contract provides an incentive for producers to harvest and
sell spot memory, it has the opposite effect on consumers,
discouraging spot-memory consumption.

Requiring a producer to compensate consumers for such early
reclamation helps remedy this concern.  If a consumer issues a
{\tt{}GET} to a producer that has evicted its value during the
agreed-upon lease period, it should not be charged for the associated
memory consumption.  An additional rebate to
compensate the consumer for its loss would provide an
incentive for the producer to avoid over-producing spot memory by
tracking the burstiness of its own memory demand.

\paragraph{Enforcement.}
Arbitrating disagreements between producers and consumers that are
potentially misbehaving presents interesting challenges, such as
determining whether a producer prematurely evicted consumer data, or
the consumer never actually stored it.  One option is to rely on a
reputation-based trust model~\cite{peertrust}, and enter into
transactions only with reputable entities. A complementary approach is
to perform lightweight probabilistic spot checks, auditing producers
to ensure they are faithfully storing consumer
data~\cite{proof-of-retrievability,storj-whitepaper}.

\paragraph{Benefit of Different Pricing Models.}

%% Moreover, the producer may be required to pay additional
%% compensatation to the consumer for its lost performance. The penalty
%% amount is specified up-front by the broker performing the match;
%% e.g. a penalty equal to the orginal charge might be reasonable.  This
%% arrangement provides an incentive for the producer to track the
%% burstiness of its demand in order to avoid over-producing spot memory.

%% \carl{Who enforces this, and how can disputes be arbitrated? For
%%   example, suppose a consumer says the producer didn't keep its
%%   key-value pair for the agreed-upon time period, but the producer
%%   says the consumer never stored it there in the first place?  One
%%   thought is to perhaps have the broker make spot checks on its own,
%%   or to introduce some reputation-based system, but both seem messy.}

%% XXX [carl] additional issues
%%
%% - consumer evict non-ghost on ghost/remote hit
%% - granularity; buy bulk, use incrementally
%% - bid/ask




==> implementation.tex <==
\section{Implementation}

\todo{May not need one depending on how we write the earlier ones.}


==> price-model.tex <==
\section{Pricing Spot Memory}
\label{sec:price-model}

Spot memory must be offered at a price that is attractive to both
producers and consumers, providing incentives to participate in the
spot-memory market.  A producer must weigh the cost of providing
memory, including the risk of transient application performance
degradation, against the monetary benefit of receiving income for
otherwise-wasted resources, which can help defray the expense of
running its own VM.  A consumer must weigh the monetary cost of
leasing spot memory against the value of its expected performance
benefit.
% from access to remote memory.

Numerous approaches inspired by microeconomics have been used to
determine prices for computational resources within individual
servers~\cite{ginseng1,ginseng2,currentcy}, distributed
systems~\cite{spawn,popcorn,g-commerce}, and the public
cloud~\cite{agmon2013deconstructing,raas,song2012optimal,zheng2015bid,xu2013dynamic,zhang2011dynamic}.
Typically, producers hold auctions designed to maximize profits, and
consumers employ bidding strategies to maximize utility.

\paragraph{Leveraging Spot-Instance Prices.}

In the public cloud, an alternative to spot memory is spinning up an
entire VM as a spot instance, and utilizing its memory
remotely~\cite{spot-cache}.  This provides a useful upper bound on the
reasonable price that can be charged for spot memory; higher prices
would present an arbitrage opportunity, making it profitable to rent
spot instances and resell their memory capacity as spot
memory.\footnote{This is analogous to breaking up a company when the
  sum of its parts is more valuable than the whole; instance CPU
  time could be resold as well.}

This observation suggests one simple method for setting a single
global price for spot memory dynamically -- without the complexity of
running separate auctions -- by leveraging price information in the
existing spot-instance market.  For example, the price for leasing $M$
MB of spot memory for $T$ minutes could be set to a fraction (such as
one-quarter) of the current cost of a spot instance for the same
duration, scaled by the ratio of $M$ to the instance's total memory
capacity.

\paragraph{Consumer Strategy.}

In general, it may be difficult for a consumer to estimate the
monetary value it should assign to additional memory.  However, when
its application is a cache, quantitative metrics can help guide this
estimate.  For example, lightweight sampling-based techniques~\cite{SHARDS,kinetic,cachesims} 
%such as
%SHARDS~\cite{SHARDS}, AET~\cite{kinetic}, or miniature
%simulation~\cite{cachesims} 
can estimate miss ratio curves (MRCs)
accurately, yielding the expected performance benefit from a larger
cache size.

The monetary value of additional cache space can be estimated by first
computing the current {\em price-per-hit} from the known cost to the
consumer of running its VM, and its observed hit rate.  The expected
increase in hits can be computed from an MRC, and valued based on the
per-hit price.  When spot memory is more valuable to the consumer than
its cost at the current market price, it should be leased, yielding an
economic consumer surplus.

The consumer must also consider the lower performance of a hit to
remote spot memory, relative to a local hit. For example, if this
increases the end-to-end latency observed by a client of the
cache significantly, the consumer may be willing to pay only a
fraction of its cost for a local hit.
% , depending on its actual QoS requirements.

%% XXX [carl] cut since too long and complex; simplified/shortened above
%%
%% Even without using MRCs, the cache can track the number of accesses to
%% a small sampled subset of its keys.  Whenever sampled entries are
%% evicted, their observed hit rates (access count divided by time
%% resident in the cache) can be smoothed to estimate the expected
%% marginal hit rate for an additional cache entry.  The monetary cost of
%% a marginal cache entry can be computed from the known price paid to
%% run the entire VM, scaled by the ratio of the size of a single entry
%% to the VM's total size.  Combining these values yields the marginal
%% {\em price-per-hit}, which can be used to decide if the current price
%% of spot-memory is attractive.\footnote{Since cache miss rates
%%   generally decrease monotonically with cache size, extrapolating from
%%   the per-entry value will overestimate the value of adding a large
%%   amount of cache space, which is better approximated using
%%   an MRC.  The {\em average} price-per-hit across the entire cache may
%%   also be useful.}  The residency time can also serve as an estimate
%% of the desired lease time to request for spot-memory allocations.

%% A similar calculation could be made to estimate the monetary cost
%% incurred for servicing a miss.

%% XXX [carl] some text about ghost buffers that might be useful
%%
%% Consider the case where the consumer is a key-value store that locally
%% stores ``proxy'' entries, as described in
%% Section~\ref{sec:security-design}.  Each proxy entry contains a key
%% and an associated value consisting of compact metadata that is used to
%% retrieve the larger actual value stored in remote spot memory.  These
%% proxy entries can also be viewed as {\em ghosts} -- small
%% metadata-only entries containing keys, but not actual values -- which
%% serve as placeholders to determine when an access would have been a
%% hit in a larger cache~\cite{tip-ghost}.

\paragraph{Early Reclamation.}

A consumer leases a fixed amount of spot memory from a producer for a
specified duration.  However, a producer may reclaim spot memory that
has been harvested from it at any time, in order to prevent
non-trivial performance degradation if its memory demand spikes.
While this contract provides an incentive for producers to harvest and
sell spot memory, it has the opposite effect on consumers,
discouraging spot-memory consumption.

Requiring a producer to compensate consumers for such early
reclamation helps remedy this concern.  If a consumer issues a
{\tt{}GET} to a producer that has evicted its value during the
agreed-upon lease period, it should not be charged for the associated
memory consumption.  An additional rebate to
compensate the consumer for its loss would provide an
incentive for the producer to avoid over-producing spot memory by
tracking the burstiness of its own memory demand.

\paragraph{Enforcement.}
Arbitrating disagreements between producers and consumers that are
potentially misbehaving presents interesting challenges, such as
determining whether a producer prematurely evicted consumer data, or
the consumer never actually stored it.  One option is to rely on a
reputation-based trust model~\cite{peertrust}, and enter into
transactions only with reputable entities. A complementary approach is
to perform lightweight probabilistic spot checks, auditing producers
to ensure they are faithfully storing consumer
data~\cite{proof-of-retrievability,storj-whitepaper}.

%% Moreover, the producer may be required to pay additional
%% compensatation to the consumer for its lost performance. The penalty
%% amount is specified up-front by the broker performing the match;
%% e.g. a penalty equal to the orginal charge might be reasonable.  This
%% arrangement provides an incentive for the producer to track the
%% burstiness of its demand in order to avoid over-producing spot memory.

%% \carl{Who enforces this, and how can disputes be arbitrated? For
%%   example, suppose a consumer says the producer didn't keep its
%%   key-value pair for the agreed-upon time period, but the producer
%%   says the consumer never stored it there in the first place?  One
%%   thought is to perhaps have the broker make spot checks on its own,
%%   or to introduce some reputation-based system, but both seem messy.}

%% XXX [carl] additional issues
%%
%% - consumer evict non-ghost on ghost/remote hit
%% - granularity; buy bulk, use incrementally
%% - bid/ask

